SAAMPLE: A Segregated Accuracy-driven Algorithm for Multiphase Pressure-Linked Equations

Existing hybrid Level Set / Front Tracking methods have been developed for structured meshes and successfully used for efficient and accurate simulations of complex multiphase flows. This contribution extends the capability of hybrid Level Set / Front Tracking methods towards handling surface tension driven multiphase flows using unstructured meshes. Unstructured meshes are traditionally used in Computational Fluid Dynamics to handle geometrically complex problems. In order to simulate surface-tension driven multiphase flows on unstructured meshes, a new SAAMPLE Segregated Accuracy-driven Algorithm for Multiphase Pressure-Linked Equations is proposed, that increases the robustness of the unstructured Level Set / Front Tracking (LENT) method. The LENT method is implemented in the Open- FOAM open source code for Computational Fluid Dynamics.

==> tables/HADAMARD_RYBCZYNSKY_2D.tex <==
\begin{tabular}{lrrrrrrr}
\toprule
{} &         H &     L\_INF &  O(L\_INF) &  EPSILON\_R\_EXACT\_MAX &  O(EPSILON\_R\_EXACT\_MAX) &  N\_CELLS &    SSUM\_PHI \\
VELOCITY\_MODEL         &           &           &           &                      &                         &          &             \\
\midrule
HADAMARD\_RYBCZYNSKY\_2D &  0.125000 &  1.423966 &  1.897036 &             1.423966 &                1.897036 &       64 &  227.858397 \\
HADAMARD\_RYBCZYNSKY\_2D &  0.062500 &  0.382327 &  1.622404 &             0.382327 &                1.622404 &      256 &  264.591468 \\
HADAMARD\_RYBCZYNSKY\_2D &  0.031250 &  0.124177 &  0.152762 &             0.124177 &                0.152762 &     1024 &  284.147454 \\
HADAMARD\_RYBCZYNSKY\_2D &  0.015625 &  0.111701 &  0.201948 &             0.111701 &                0.201948 &     4096 &  294.221861 \\
HADAMARD\_RYBCZYNSKY\_2D &  0.007813 &  0.097110 &  0.062653 &             0.097110 &                0.062653 &    16384 &  299.333072 \\
HADAMARD\_RYBCZYNSKY\_2D &  0.003906 &  0.092983 &  0.062653 &             0.092983 &                0.062653 &    65536 &  301.907169 \\
\bottomrule
\end{tabular}


==> tables/SHEAR_2D.tex <==
\begin{tabular}{lrrrrrrr}
\toprule
{} &         H &     L\_INF &  O(L\_INF) &  EPSILON\_R\_EXACT\_MAX &  O(EPSILON\_R\_EXACT\_MAX) &  N\_CELLS &      SSUM\_PHI \\
VELOCITY\_MODEL &           &           &           &                      &                         &          &               \\
\midrule
SHEAR\_2D       &  0.125000 &  0.032961 &  1.833407 &             0.032961 &                1.833407 &       64 &  3.885781e-15 \\
SHEAR\_2D       &  0.062500 &  0.009249 &  1.955529 &             0.009249 &                1.955529 &      256 &  1.665335e-14 \\
SHEAR\_2D       &  0.031250 &  0.002385 &  1.988745 &             0.002385 &                1.988745 &     1024 &  3.663736e-14 \\
SHEAR\_2D       &  0.015625 &  0.000601 &  1.997178 &             0.000601 &                1.997178 &     4096 &  8.881784e-14 \\
SHEAR\_2D       &  0.007813 &  0.000150 &  1.999294 &             0.000150 &                1.999294 &    16384 &  1.421085e-13 \\
SHEAR\_2D       &  0.003906 &  0.000038 &  1.999294 &             0.000038 &                1.999294 &    65536 &  3.552714e-13 \\
\bottomrule
\end{tabular}

